Backward CUSUM for Testing and Monitoring Structural Change with an Application to COVID-19 Pandemic Data

It is well known that the conventional cumulative sum (CUSUM) test suffers from low power and large detection delay. In order to improve the power of the test, we propose two alternative statistics. The backward CUSUM detector considers the recursive residuals in reverse chronological order, whereas the stacked backward CUSUM detector sequentially cumulates a triangular array of backwardly cumulated residuals. A multivariate invariance principle for partial sums of recursive residuals is given, and the limiting distributions of the test statistics are derived under local alternatives. In the retrospective context, the local power of the tests is shown to be substantially higher than that of the conventional CUSUM test if a break occurs in the middle or at the end of the sample. When applied to monitoring schemes, the detection delay of the stacked backward CUSUM is found to be much shorter than that of the conventional monitoring CUSUM procedure. Furthermore, we propose an estimator of the break date based on the backward CUSUM detector and show that in monitoring exercises this estimator tends to outperform the usual maximum likelihood estimator. Finally, an application of the methodology to COVID-19 data is presented.

==> 3_backwardCUSUM_tests.tex <==
\section{Backward CUSUM R-test} \label{sec:backCUSUM}

\begin{table}[t]
\caption{Asymptotic critical values for $\mathcal{Q}_T$ and $\mathcal{BQ}_T$}
\centering
\begin{footnotesize}
\begin{tabular}{l|llllllll}
 & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$ & $k=6$ & $k=7$ & $k=8$ \\ \hline
 $\alpha = 1\%$ & 1.143 & 1.219 & 1.260 & 1.287 & 1.307 & 1.323 & 1.338 & 1.349 \\
 $\alpha = 5\%$ & 0.945 & 1.032 & 1.081 & 1.114 & 1.139 & 1.160 & 1.176 & 1.189 \\
 $\alpha = 10\%$& 0.847 & 0.941 & 0.993 & 1.029 & 1.056 & 1.077 & 1.095 & 1.110 \\ \hline \hline
\end{tabular}
\end{footnotesize}
\hspace*{0.1ex}
\parbox{11.9cm}{ \vspace{0.5ex} \spacingset{1} \scriptsize
Note: Simulated $(1-\alpha)$ quantiles of $\sup_{r \in [0,1]} \| W^{(k)}(r)\|/(1+2r)$ based on 100,000 Monte Carlo replications are reported. 
The Wiener process is approximated on a grid of 10,000 equidistant points.
}
\label{tab_crit1}
\end{table}


An alternative approach is to cumulate the recursive residuals in reversed order.
Suppose there is a single break in $\beta_t$ at time $t=T^*$.
Then, $\{ w_t, \ t < T^* \}$ are the residuals from the pre-break period, and $\{ w_t, \ t \geq T^* \}$ are those from the post-break period.
As the pre-break recursive residuals are not affected by a violation of the null hypothesis, they do not provide useful information about a subsequent break. Accordingly, the partial sum process $T^{-1/2} \sum_{j=1}^t w_j$ behaves like a pure random walk for $t < T^*$ and cumulating those residuals brings nothing but noise to the detector statistic. In contrast, the post-break residuals have nonzero mean and reveal relevant information about a possible break. In order to focus on the post-break residuals, we therefore consider backwardly cumulated partial sums of the form $T^{-1/2} \sum_{j=0}^{t-1} w_{T-j}$. We define the retrospective backward CUSUM detector as
\begin{equation*}
	BQ_{t,T} = Q_T(1) - Q_T\big(\tfrac{t-1}{T}\big) = \frac{1}{\widehat \sigma_T \sqrt{T}} C_T^{-1/2} \sum_{j=t}^T x_j w_j	\quad (t=1, \ldots, T).
\end{equation*}
The null hypothesis is rejected if $\|BQ_{t,T}\|$ exceeds the boundary
$b_t = b((T-t-1)/T)$ for at least one time index $t$.

\begin{theorem} \label{thm:backwardCUSUM}
Let $g(r)$ be piecewise constant and bounded, and let $\beta_t = \beta_0 + T^{-1/2} g(t/T)$ for all $t \in \mathbb{N}$.
Then, under Assumptions \ref{assumption}--\ref{ass:boundary}, as $T \to \infty$,
\begin{equation*}
	\mathcal{BQ}_T = \max_{t= 1, \ldots, T} \|BQ_{t,T}\|/ d\big(\tfrac{T-t+1}{T}\big) \Dlim  \sup_{r \in [0,1]} \| W^{(k)}(r) + C^{1/2} (h(1) - h(1-r)) \|/d(r).
\end{equation*}
\end{theorem}

\noindent
The limiting distributions of $\mathcal{Q}_T$ and $\mathcal{BQ}_T$ coincide under $H_0$ and differ under the alternative.
A simple illustrative example of the detector paths together with the linear boundary \eqref{linearboundary} of \cite{brown1975} are depicted in Figure \ref{fig_motivation}, in which a process with $k=1$ and a single break in the mean at $3/4$ of the sample is simulated.
Simulated asymptotic critical values are presented in Table \ref{tab_crit1}.

\begin{figure}[t]
\centering
\caption{Illustrative example for the backward CUSUM with a break in the mean}
\includegraphics[scale=0.34]{./img/figure2.pdf}
\hspace*{0.5ex}
\parbox{14cm}{ \spacingset{1} \scriptsize
Note: The process $y_t = \mu_t + u_t$, $t=1, \ldots, T$, is simulated for $T=100$ with $\mu_t = 0$ for $t < 75$, $\mu_t = 1$ for $t \geq 75$, and $u_t \sim NID(0,1)$.
The bold solid line paths are the trajectories of $\|Q_{t,T}\|$ and $\|BQ_{t,T}\|$, where the detectors are univariate such that the norm is just the absolute value.
In the background, the recursive residuals are plotted.
The dashed lines correspond to the linear boundary \eqref{linearboundary} with significance level $\alpha = 5\%$ and critical value $\lambda_\alpha = 0.945$.
}
\label{fig_motivation}
\end{figure}





\section{Stacked backward CUSUM R- and M-tests} \label{sec:stackbackCUSUM}

Unlike the forward CUSUM detector, the backward CUSUM detector is not measurable with respect to the filtration of available information at time $t$ and is therefore not suitable for a monitoring procedure.
The path of $\|BQ_{t,T}\|$ is only defined for $t \leq T$, as its endpoint $T$ is fixed.
To combine the advantages of $BQ_{t,T}$ with the measurability properties of $Q_{t,T}$,
we resort to an inspection scheme, which goes back to \cite{page1954} and involves a triangular array of residuals.
Let $\mathcal{BQ}_T(t) = \max_{s=1, \ldots, t} \|Q_T(t/T) -  Q_T((s-1)/T)\|/d((t-s+1)/T)$
be the backward CUSUM statistic with endpoint $t$.
The idea is to compute this statistic sequentially for each time point, yielding
$\mathcal{BQ}_T(1), \ldots, \mathcal{BQ}_T(T)$.
The stacked backward CUSUM statistic is the maximum among this sequence of backward CUSUM statistics.
An important feature of this sequence is that it is measurable with respect to the filtration of information at time $t$, so that $\mathcal{BQ}_T(t)$ is itself a sequential statistic.
Stacking all backward CUSUM statistics on one another leads to a triangular array structure given by
%The stacked backward CUSUM detector is defined as
	\begin{equation*}
		SBQ_{s,t,T} =  Q_T\big(\tfrac{t}{T}\big) -  Q_T\big(\tfrac{s-1}{T}\big) = \frac{1}{\widehat \sigma_T \sqrt{T}} C_T^{-1/2}\sum_{j=s}^t x_j w_j \quad  (t \in \mathbb N, \ s=1, \ldots, t),
	\end{equation*}
which is denoted as the stacked backward CUSUM detector.
We reject $H_0$ if $\|SBQ_{s,t,T}\|$ exceeds the two-dimensional boundary $b_{s,t} = b((t-s+1)/T)$ for some $t=1, \ldots, T$ and $s = 1, \ldots, t$.
Equivalently, $H_0$ is rejected if the double maximum statistic
\begin{equation*}
	\mathcal{SBQ}_T = \max_{t=1, \ldots, T} \mathcal{BQ}_T(t) = \max_{t=1, \ldots, T} \max_{s=1, \ldots, t} \| SBQ_{s,t,T} \| / d( \tfrac{t-s+1}{T} )
\end{equation*}
exceeds $\lambda_\alpha$.
The triangular detector can also be monitored on-line across all the time points $t > T$.
The null hypothesis is rejected if $\|SBQ_{s,t,T}\|$ exceeds $b_{s,t} = b((t-s+1)/T )$ at least once for some $t \geq T+1$ and $s = T+1, \ldots, t$.
Analogously to the retrospective case, let
\begin{equation*}
	\mathcal{SBQ}_{T,m} = \max_{t=T+1, \ldots, \mT} \max_{s=T+1, \ldots, t} \| SBQ_{s,t,T} \| / d( \tfrac{t-s+1}{T} )
\end{equation*}
be the maximum statistic for fixed endpoint monitoring.

\begin{theorem} \label{thm:stackedbackwardCUSUM}
Let $g(r)$ be piecewise constant and bounded, let $\beta_t = \beta_0 + T^{-1/2} g(t/T)$ for all $t \in \mathbb{N}$, and let $m < \infty$.
Then, under Assumptions \ref{assumption} and \ref{ass:boundary}, as $T \to \infty$,
\begin{align*}
	\mathcal{SBQ}_T &\Dlim  \sup_{r \in [0,1]} \sup_{s \in [0,r]} \| W^{(k)}(r) - W^{(k)}(s) + C^{1/2} [h(r) - h(s)] \|/d(r-s), \\
	\mathcal{SBQ}_{T,m} &\Dlim  \sup_{r \in [0,m-1]} \sup_{s \in [0,r]} \| W^{(k)}(r) - W^{(k)}(s) + C^{1/2} [h(r+1) - h(s+1)] \|/d(r-s).
\end{align*}
\end{theorem}


Simulated critical values for the stacked backward CUSUM $R$- and $M$- tests are presented in Table \ref{tab_crit3}.



\begin{table}[t]
\caption{Asymptotic critical values for $\mathcal{SBQ}_{T}$ and $\mathcal{SBQ}_{T,m}$}
\centering
\begin{footnotesize}
\begin{tabular}{l|cccccccccccc}
 & \multicolumn{3}{c}{$k=1$} & \multicolumn{3}{c}{$k=2$} & \multicolumn{3}{c}{$k=3$} & \multicolumn{3}{c}{$k=4$} \\ \hline
$m$ \textbackslash \ $\alpha$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ \\
1.2 & 0.782 & 0.859 & 1.024 & 0.859 & 0.935 & 1.092 & 0.902 & 0.975 & 1.129 & 0.932 & 1.003 & 1.152 \\ 
1.4 & 0.941 & 1.030 & 1.208 & 1.028 & 1.111 & 1.277 & 1.076 & 1.156 & 1.320 & 1.108 & 1.185 & 1.345 \\ 
1.6 & 1.026 & 1.113 & 1.292 & 1.111 & 1.192 & 1.365 & 1.158 & 1.238 & 1.406 & 1.189 & 1.269 & 1.432 \\ 
1.8 & 1.077 & 1.162 & 1.344 & 1.161 & 1.244 & 1.411 & 1.208 & 1.286 & 1.452 & 1.240 & 1.317 & 1.476 \\ 
2 & 1.113 & 1.198 & 1.374 & 1.196 & 1.277 & 1.442 & 1.244 & 1.321 & 1.481 & 1.275 & 1.350 & 1.506 \\ 
4 & 1.262 & 1.339 & 1.500 & 1.336 & 1.410 & 1.564 & 1.378 & 1.450 & 1.599 & 1.407 & 1.478 & 1.621 \\ 
10 & 1.367 & 1.440 & 1.588 & 1.437 & 1.503 & 1.644 & 1.475 & 1.540 & 1.677 & 1.500 & 1.565 & 1.703 \\ 
%$\infty$ & 1.450 & 1.514 & 1.648 & 1.512 & 1.573 & 1.703 & 1.547 & 1.606 & 1.736 & 1.570 & 1.629 & 1.760 \\ \hline
 & \multicolumn{3}{c}{$k=5$} & \multicolumn{3}{c}{$k=6$} & \multicolumn{3}{c}{$k=7$} & \multicolumn{3}{c}{$k=8$} \\ \hline
$m$ \textbackslash \ $\alpha$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ & $10\%$ & $5\%$ & $1\%$ \\
1.2 & 0.954 & 1.023 & 1.170 & 0.972 & 1.041 & 1.186 & 0.987 & 1.054 & 1.198 & 1.000 & 1.065 & 1.206 \\ 
1.4 & 1.133 & 1.208 & 1.366 & 1.152 & 1.225 & 1.381 & 1.167 & 1.241 & 1.396 & 1.181 & 1.253 & 1.409 \\ 
1.6 & 1.214 & 1.293 & 1.452 & 1.235 & 1.311 & 1.466 & 1.251 & 1.325 & 1.477 & 1.265 & 1.339 & 1.488 \\ 
1.8 & 1.265 & 1.340 & 1.496 & 1.283 & 1.357 & 1.511 & 1.300 & 1.372 & 1.525 & 1.315 & 1.385 & 1.537 \\ 
2 & 1.299 & 1.372 & 1.526 & 1.317 & 1.388 & 1.541 & 1.333 & 1.404 & 1.556 & 1.347 & 1.418 & 1.566 \\ 
4 & 1.429 & 1.497 & 1.638 & 1.446 & 1.513 & 1.651 & 1.461 & 1.527 & 1.665 & 1.473 & 1.539 & 1.679 \\ 
10 & 1.520 & 1.584 & 1.718 & 1.536 & 1.599 & 1.732 & 1.551 & 1.612 & 1.744 & 1.562 & 1.623 & 1.752 \\ 
%$\infty$ & 1.589 & 1.647 & 1.775 & 1.604 & 1.661 & 1.788 & 1.617 & 1.673 & 1.799 & 1.627 & 1.683 & 1.807 \\ \hline \hline
\end{tabular}
\end{footnotesize}
\hspace*{0.1ex}
\parbox{15.9cm}{ \vspace{0.5ex} \spacingset{1} \scriptsize
Note: Simulated $(1-\alpha)$ quantiles of $\sup_{r \in [0,1]} \sup_{s \in [0,r]} \| W^{(k)}(r) - W^{(k)}(s)\|/(1+2(r-s))$ based on 100,000 Monte Carlo replications are reported. The critical values for $\mathcal{SBQ}_{T}$ are the same as those for $\mathcal{SBQ}_{T,m}$ with $m=2$.
}
\label{tab_crit3}
\end{table}



\begin{remark} \label{rem:partial}
In practice one is often interested in breaks in certain coefficients or directions.
Partial or one-sided tests can be beneficial in terms of a more powerful test.
For testing the partial hypothesis $H_0: H' \beta_t = H' \beta_0$, where $H$ is an orthonormal $k \times l$ matrix, consider the partial CUSUM process $Q_T^*(t/T) = Q_{t,T}^* = \widehat \sigma_T^{-1} T^{-1/2} (H' C_T H)^{-1/2} H' \sum_{j=1}^t x_j w_j$.
Then, $H_0$ is rejected if $\| Q_{t,T}^* - Q_{s,T}^* \|$ (partial SBQ test) or $\| Q_{T,T}^* - Q_{t,T}^* \|$ (partial BQ test) exceeds the respective boundary.
Note that the critical values for the $l$-dimensional CUSUM test from Tables \ref{tab_crit1} and \ref{tab_crit3} can be applied for the partial test, since $Q_T^*(r) \Rightarrow W^{(l)}(r)$ under $H_0$.
%
When testing against the one-sided alternative $H' \beta_t > H' \beta_0$, we reject if $p(H' BQ_{t,T})$ or $p(H' SBQ_{s,t,T})$ exceeds the respective boundary function, where $p(x) = \max_{i=1, \ldots, l} x_i$, $x \in \mathbb R^l$.
The critical value coincides with the $(1-2\alpha)$ quantile of the respective $l$-dimensional limiting process.
For instance, when testing for positive breaks in the intercept with $\alpha = 5\%$, the retrospective stacked backward CUSUM rejects
if $p(H' SBQ_{s,t,T})$ exceeds $1.113 \cdot d((t-s+1)/T)$.
\end{remark} 
